Learn from Your Neighbor: Learning Multi-modal Mappings from Sparse Annotations

Many structured prediction problems (particularly in vision and language domains) are ambiguous, with multiple outputs being correct for an input - e.g. there are many ways of describing an image, multiple ways of translating a sentence; however, exhaustively annotating the applicability of all possible outputs is intractable due to exponentially large output spaces (e.g. all English sentences). In practice, these problems are cast as multi-class prediction, with the likelihood of only a sparse set of annotations being maximized - unfortunately penalizing for placing beliefs on plausible but unannotated outputs. We make and test the following hypothesis - for a given input, the annotations of its neighbors may serve as an additional supervisory signal. Specifically, we propose an objective that transfers supervision from neighboring examples. We first study the properties of our developed method in a controlled toy setup before reporting results on multi-label classification and two image-grounded sequence modeling tasks - captioning and question generation. We evaluate using standard task-specific metrics and measures of output diversity, finding consistent improvements over standard maximum likelihood training and other baselines.

==> sections/formulation.tex <==
% Consider a dataset $\calD \in \calX \times \calY$ consisting of inputs $\xb \in \calX$ and corresponding outputs $\yb \in \calY$. 
% Further the dataset has structure such that we observe some function $f(\cdot)$ of a set of inputs  $X = \{\xb_1, \xb_2, \dots \xb_f\}$ and a corresponding aggregation of their outputs \ie $g(Y)$ where $Y = \{\yb_1, \yb_2, \dots \yb_f\}$.
% For image-captioning, the elements of $X$ would correspond to different spatial (or semantic) divisions of the image and elements of $Y$ are corresponding words or phrases.
% The unknown aggregating functions $f,g$ coherently bring together the various parts to form meaningful images or sentences.

% \textbf{Problem 1.} Given such a dataset, can we generate captions for new images ? 
% This will require learning the functions $f^{-1}$ and $g$.
% A CNN can be thought of learning $f^{-1}$ where the $fc5$ or $fc7$ features can represent spatial / semantic divisions of the input.
% \\ \\
% \subsection{Loss}
Let us assume that each image $X^{(i)}$ is a set of (indenpendent?) spatial or semantic collection of objects \ie $X^{(i)} = \{\xb_1^{(i)}, \xb_2^{(i)}, \dots \xb_k^{(i)}\}$.
For example, if we use a standard CNN like VGG, the fc5 layer can be thought of as decomposing the image into $14\times14$ (512-dimensional) vectors that contain the semantic information of the image.
    Similarly, the corresponding caption (the language component) can be thought of as  collections of objects \ie $Y^{(i)} = \{\hb_{1}^{(i)}, \dots \hb_T^{(i)}\}$ where $\hb_t^{(i)}$ represents the encoding of the sequence up to time $t$. (these instances are probably not independent -- they are Markovian since history encodings are stateful...)
    So, each data point is essentially a ``bag" (from multiple instance learning) that consists of both visual and language isntances. Let us denote each such data point as $B^{(i)} = \{X^{(i)}, Y^{(i)}\}$.
\\ \\
        \emph{Purely} visual attention models consider a bag (drawing from the connection between MIL and attention mechanism) consisting of only the image features. 
    In a similar vein, \cite{lu_cvpr17} alter this bag to be ``multi-modal" \ie it now also includes language information in the form of the current hidden state.
    Note that by definition the instances of a bag compete with each other.
\\ \\
Now, consider a graph on these data-points -- where edges between bags are a result of edges between both the visual and language ``instances" and hence, its corresponding weight.
There is also a temporal component in that the attention on the visual features and the hidden state are time-dependent. 
In that sense, the weight of the edges between two data-points needs to be re-computed at each step -- which is the nature of ``applicability''.
\ak{We can think of this as attending to neighbors dynamically.} \\ \\
From a top-down perspective -- Our problem is an interesting case where each datapoint has two aspects -- visual and lingual where both are structured data with different dependencies between their ``sub-structures''.
    These sub-structures are like atoms of a dictionary that can be used to \emph{compose} a datapoint. 
    Given a correspondence between two structures, we want to figure out relationships between their  sub-structures while also jointly learning them. 
    Naturally, given access to oracle functions that decide how each modality composes the substructures and the applicability function that decides the correspondence between sub-structures (\ak{mapping between the two composing functions}) our problem is straight-forward to solve.

\textbf{Applicability:} We assume that the sub-structures or the instances that form the bag are learnt efficiently by the very design of CNNs and RNNs for vision and language respectively.
So, let us define applicability as a product of both (dynamic) visual and language similarity \ie 
\[w_t(B^{(i)}, B^{(j)}) = \calS_v(X^{(i)}, X^{(i)}) \ \calS_{\ell}(Y^{(i)},Y^{(j)})\]
We want the applicability function to decide if the neighbor should play any rule in the prediction of the next token -- naturally, this means that both the similarites are contextual.
Visual similarity is given by:
\[\calS_v(X^{(i)}, X^{(j)}) = \max_{k\in [K]} \iprod{\tilde{\xb}^{(i)}}{\xb_k^{(j)} } \]
where $\tilde{\xb}^{(i)} = \sum_k \alpha_k \xb_k^{(i)}$ is the attended image vector at time $t$ and $K$ is the number of visual instances in each image. (\ak{(a) I think $\max$ is just one form of aggregation -- intuitively made more sense than average. We can think of having an MLP there instead, etc. (b) Leaving out time from the equations for now -- all these similarities ARE time-dependent}). \\ \\
In words -- if what the model is looking at right now has some other region in a neighboring image that is very similar, then the visual similarity is high. \\ \\
Language Similarity is also defined in a similar manner \ie it is high if the current hidden state correlates to \emph{any} hidden-state of a neighboring caption. Additionally, we also save that time step of the neighboring caption to be able to copy over the language.
\[\calS_{\ell}(Y^{(i)}, Y^{(j)}) = \max_{k\in [T]} \iprod{\hb^{(i)}_t}{\hb_k^{(j)}} \]
\[\tau = \argmax_{k\in [T]} \iprod{\hb^{(i)}_t}{\hb_k^{(j)}} \]
So, the objective at each time step has (a) the conventional log-likelihood term \ie
\[\calL_{CE} = \log Pr(y_t = y^{(i)}_t \ | \ \hb^{(i)}_{t-1}, X^{(i)}) \]
(b) the ``copy'' over term:
\[\calL_{N} = w(B^{(i)}, B^{(j)}) \log Pr(y_t = y^{(j)}_{\tau} \ | \ \hb_{t-1}^{(i)}, X^{(i)})\]
So, the loss is:
\[\calL_{CE} + \lambda \calL_N\]

So, we are saying -- if we find some semantic concept that are similar AND find some part of the sentence also relevant, only then copy over.

Regularization:

All the parameters are shared \ie there is only one CNN and one RNN -- so, that should effectively act as a regularizer. 
If the model still has capacity to push each and every instance of a concept apart (tell difference between this red pand and that red panda, highly unlikely), we will need to add constraints that encode priors (like we did for $K_{ij}$ using $\mu$) on the entire sequence of applicability weights -- only some of them can be small or zero.

\textbf{Compositionality comes at a cost:} \\
Composition in both vision and language is taken into account since at every step the model is free to chose from \emph{any} part of the neighboring image and \emph{any} part of the neighboring caption.
So, apart from the cost of attention, we also have the additional cost of looking at the neighboring image making it -- $\calO(n^2KT)$ where $n$ is the number of instances in the visual bag, K is the number of nearest neighbors and $T$ the number of time steps.
The language part need not have any self-attention and hence is $\calO(mTK)$ where $m$ is the number of words in the neighboring caption and the other symbols have the same meaning.

Why I like this formulation:
\begin{itemize}
        \item Gets rid of the multipliers within the actual log-likelihood term which were mathematically unintuitive.
        \item Comes closer to our initial label-smoothing formulation -- Essentially we just add label noise at each time-step by forcing to predict other words as well.
        \item We reason at each time step -- so, compositionality comes more naturally. Hopefully, if the model picks up basic visual features and language constructs the applicability function will not output junk.
        \item The applicability function is closer to multimodal distributional semantics -- similar internal states must be able to predict words that occur in similar contexts.
            This way, we need not worry about alignment -- If the $h_{t+1}$ is similar to the neighbor's caption the method will force $\tau+1$ word to be copied as well. 
            This way arbitrary length copies are possible as against making independent word-level decisions.
        \item Although the details concern vision and language, the MIL intuitions show the way forward to extend this approach to other types of multi-modal tasks or data.
            As long as you have a way to figure out the instances that form the bag and the right sort of ``priors'' that decide the applicability function, you are good! 
\end{itemize}

I am not sure if we need to include the language component in the self-attention (like \cite{lu_cvpr17}) -- we can try both out starting from visual-only attention.
My bets are that we would not need this since we are interested in copying over words that are ALSO grounded in vision.
\\ \\ 
\textbf{Smoothing}
A common type of smoothing term between two ``similar'' instances is: 
\[\lambda \norm{f(\xb_1) - f(\xb_2)}\]
Instead in our approach, we have a term that goes as 
\[\lambda \norm{\yb_2 - f(\xb_1)}\]
Since, we are also minimizing $\norm{\yb_2 - f(\xb_2)}$, are these two smoothing techniques equivalent ? Or are there any advantages of one over the other ?

% The loss for each point is:
% \begin{equation} 
    % \calL_i = \ell_{ii} + \frac{\lambda}{N{-}1} \sum_j K_{ij}\ell_{ij} + \frac{\mu}{N{-}1} \sum_j (K_{ij}{-}1)^2 \nonumber
% \end{equation}
% where $\ell_{ij}$ is the NLL of $\yb_j$ conditioned on image $\xb_i$ given as:
% \[\ell_{ij} = -\frac{1}{T}\sum_{t=1}^T\log \prob(y_{j,t} | y_{j,t-1}, y_{j,t-2}, \dots y_{j,1}, \xb_i)\]
% From previous discussion, the $\lambda$ term is modified to be:
% \[-\frac{1}{N{-}1} \sum_j \sum_{t=1}^T a_{j,t} \log \prob(y_{j,t} | y_{j,t-1}, \dots y_{j,1}, \xb_i)\]
% where $a_{j,t}$ (\wrt $i$ is implicit) is the \emph{applicability} of the $t^{th}$ word of $y_j$ to image $\xb_i$.
% \ak{
% \begin{itemize}
    % \item What do the multipliers $a_{j,t}$ mean in the NLL ? In the probability space, it corresponds to exponentiating which seems weird to me.
        % One work around would be to make these multipliers binary -- if the token is not visually grounded we do not pay any loss.
    % \item The next concern is alignment -- we are copying over ``language'' but not the context/grammar since we are making these applicability decisions at the word level.
    % \item Jiasen's captioning model computes attention over some $K$ visual features and one language feature -- resulting in a probability distribution over $K{+}1$ elements.
        % So, the multiplier $a_{j,t}$ is: $1-\alpha_{K{+}1}$ \ie the sum of attention on all visual features.
        % Since what is ``visually grounded'' and what is coming from the language model is implicitly learnt, there is no reliability in what the model might consider visually grounded.
        % Further, the repulsive nature of the loss can easily offload most of the learning to the language model so that these multipliers are small.
        % One way to fix this might be to compute similarity in the attended feature space and then imposing the constraint that this similarity should not deviate too much from 1 (basically, the $\mu$ term).
% \end{itemize}
% \emph{Vague thoughts:} Other than this formulation, I have been thinking if our problem can be cast into a multiple instance learning setting.
% The input is a ``bag'' of spatial/semantic regions and the output is another bag of corresponding language descriptions.  
% While we get to only observe some unknown function of these two bags, the problem is to both learn the instances that make up these bags and the correspondence (or applicability) function between instances of these two bags.
% }
% \\ \\
% \ak{
% Another vague thought is to revisit probabilistic relational models (Ben Taskar and some other people) and see if any approach from that space can be DL-ed.
% }



